Temporal Enhanced Floating Car Observers

Floating Car Observers (FCOs) are an innovative method to collect traffic data by deploying sensor-equipped vehicles to detect and locate other vehicles. We demonstrate that even a small penetration rate of FCOs can identify a significant amount of vehicles at a given intersection. This is achieved through the emulation of detection within a microscopic traffic simulation. Additionally, leveraging data from previous moments can enhance the detection of vehicles in the current frame. Our findings indicate that, with a 20-second observation window, it is possible to recover up to 20\% of vehicles that are not visible by FCOs in the current timestep. To exploit this, we developed a data-driven strategy, utilizing sequences of Bird's Eye View (BEV) representations of detected vehicles and deep learning models. This approach aims to bring currently undetected vehicles into view in the present moment, enhancing the currently detected vehicles. Results of different spatiotemporal architectures show that up to 41\% of the vehicles can be recovered into the current timestep at their current position. This enhancement enriches the information initially available by the FCO, allowing an improved estimation of traffic states and metrics (e.g. density and queue length) for improved implementation of traffic management strategies.

==> images/multi_images/qualitative_results.tex <==
\begin{figure*}[hb]
    \centering
        \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/qualitative_results/arrow_6s.png}
    \end{minipage}
    \vspace{0cm}
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/input_10603.png}
        %\caption*{Caption 1}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/input_10604.png}
        %\caption*{Caption 2}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/input_10605.png}
        %\caption*{Caption 3}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/input_10606.png}
        %\caption*{Caption 4}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/input_10607.png}
        %\caption*{Caption 5}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/input_10608.png}
        %\caption*{Caption 6}
    \end{minipage}%
    \vspace{0.02cm}  % Adjust vertical spacing between rows

    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/prediction_10608_3DCNN_add.png}
        \caption*{3D CNN}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/prediction_10608_2DCNN_add.png}
        \caption*{2D CNN}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/prediction_10608_ConvLSTM_add.png}
        \caption*{Conv LSTM}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/prediction_10608_LSTM_add.png}
        \caption*{ETD-LSTM}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/prediction_10608_Transformer_add.png}
        \caption*{ETD-Transformer}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_results/target_10608.png}
        \caption*{Ground Truth}
    \end{minipage}%

    \caption{Example sequence $S$ with $s=5s$ as input into the model architectures in the first row. The second row shows the ground truth $G$ for $t$, presents the model-generated outputs $O$ from various proposed models, and highlights the lost vehicles (red), not recovered vehicles (violet), and successfully recovered vehicles (green).}
    \klaus{bin mit dieser Grafik noch nicht ganz  happy .... die oberen snapshots sind ja Eingangsgröße in die unterschiedlichen Modelle unten und sollen möglichst die ground truth ganz recht treffen, das kommt noch nicht intuitiv raus hier, auch der Begriff unhidden ist irgendwie noch nicht perfekt}
    \label{img: results}

%\klaus{figure 5 ist noch nicht ideal ... oben ggf die Sekunden dazu unten auch irgendwie mit rot/grün Treffer und Fehler markieren??? Der Pfeil soll wohl die Zeit darstellen - beschriften?}
\end{figure*}
%Results are for 10608
